Newton-Raphson Flow for Aggressive Quadrotor Tracking Control

We apply the Newton-Raphson flow tracking controller to aggressive quadrotor flight and demonstrate that it achieves good tracking performance over a suite of benchmark trajectories, beating the native trajectory tracking controller in the popular PX4 Autopilot. The Newton-Raphson flow tracking controller is a recently proposed integrator-type controller that aims to drive to zero the error between a future predicted system output and the reference trajectory. This controller is computationally lightweight, requiring only an imprecise predictor, and achieves guaranteed asymptotic error bounds under certain conditions. We show that these theoretical advantages are realizable on a quadrotor hardware platform. Our experiments are conducted on a Holybrox x500v2 quadrotor using a Pixhawk 6x flight controller and a Rasbperry Pi 4 companion computer which receives location information from an OptiTrack motion capture system and sends input commands through the ROS2 API for the PX4 software stack.

==> 0b_keywords.tex <==
newton-raphson, nonlinear control, quadrotor, ROS2, pixhawk

==> 3_Model_PRed.tex <==
The Newton-Raphson flow controller requires  a predictor for the system. In this section, we propose a simple predictor constructed from a small-angle approximation of the quadrotor dynamics. The motivation for choosing this predictor is that this simplified modeling assumption is common for tuning PID controllers and for developing controllers appropriate for nonaggressive tracking \cite{PID_Quad_Survey}. As we will see below, even with this imperfect predictor, we achieve notable tracking results. A full comparison of possible predictor methods, including those using high fidelity nonlinear or neural network models, is the subject of ongoing work. 

We take as the system state 
\begin{align}
{x} &= \begin{bmatrix}
        p_x & p_y & p_z & V_x & V_y & V_z & \phi & \theta & \psi
    \end{bmatrix}^T\in\mathbb{R}^9
\end{align}
where $(p_x,p_y,p_z)$ is the quadrotor's 3D position in a fixed world frame, $(V_x,V_y,V_z)$ is the quadrotor velocity in this frame, and ($\phi, \theta, \psi)$ are the quadrotor roll, pitch, and yaw angles. 

The system input is $u=\begin{bmatrix}u_\tau&u_p&u_q&u_r\end{bmatrix}^T\in\mathbb{R}^4$, consisting of three angular velocities $(u_p,u_q,u_r)$ and net thrust $u_\tau$ through the center of mass in the direction perpendicular to the plane of the rotors. The PX4 control architecture includes an off-board control mode that converts these inputs directly to commanded rotor velocities for the four rotor motors.

We take as the system output 
\begin{align}
y=Cx=\begin{bmatrix}p_x&p_y&p_z&\psi\end{bmatrix}^T\in\mathbb{R}^4
\end{align} for appropriately defined binary matrix $C\in\mathbb{R}^{4\times 9}$ (the detailed structure of $C$ is provided in the Appendix).

% PUT FULL A AND B MATRICES IN APPENDIX, FOR ARXIV
\subsection{Simplified Predictor Dynamics}\label{subsec:simplified predictor dynamics}
Even though we wish to control the quadrotor in aggressive regimes, to build a computationally simple predictor, we approximate the dynamics with a classical small-angle approximation and linearize at hover. The resulting dynamics used for the predictor are
\begin{align}
\label{simpleQuadDyn1}
(\dot{p}_x,\dot{p}_y,\dot{p}_z)&=(V_x,V_y,V_z)\\
\label{simpleQuadDyn2}
(\dot{\phi},\dot{\theta},\dot{\psi})&=(u_p,u_q,u_r)\\
\label{simpleQuadDyn3}
(\dot{V}_x,\dot{V}_y,\dot{V}_z)&= \left(-g\phi, g\theta, \frac{u_\tau}{m}-g\right)
\end{align}
where $m$ is the quadrotor mass and $g$ is the acceleration due to gravity. The simplified dynamics for prediction are linear and of the form $\dot{{x}}=A{x}+Bu$ for appropriate matrices $A$ and $B$, where the matrices $A$ and $B$ are defined in the Appendix.

Given state ${x}(t)$ and input $u(t)$ at time $t$, we take as the predicted state at time $t+T$ the solution to the simplified dynamics 
\begin{align}
    {x}(t+T)&=e^{AT}{x}(t) +\int _{0}^T \, e^{ A(T-\tau)}B u(t)d\tau  \\
\label{eqn:predictor2}
    &= \Tilde{A}{x}(t) + \Tilde{B} u(t)
\end{align}
for appropriate $\Tilde{A}$ and $\Tilde{B}$ that depend only on $T$ and are computable offline in closed-form. Note that, in constructing a predictor, we do not know the value of $u(\tau)$ during the duration of the lookahead period $\tau \in [t,t+T]$, and instead only know its value at the beginning of the period $\tau=t$. Therefore, we adopt a zero-order hold on the input, assuming it remains constant over the prediction horizon. We therefore obtain the final form for the predictor as
\begin{align}
\label{eq:rho}
    \hat{y}(t+T)=\rho(x(t),u(t))=C\tilde{A}x(t)+C\tilde{B}u(t)
\end{align}
where $\tilde{A}$, $\tilde{B}$, and $C$ are fixed throughout and computed as described above.





% In this section, we 

% demonstrate the quadrotor model we use for prediction, as well as its inputs and the output states we define trajectories for, and the output predictor we use to track those trajectories.

% \subsection{Quadrotor Model}
% We use a 9-dimensional quadrotor model which takes thrust and body rates as inputs. Our full system dynamics take the following form,

% \begin{align}
%     \Bar{x} &= \begin{bmatrix}
%         x & y & z & V_x & V_y & V_z & \phi & \theta & \psi
%     \end{bmatrix}^T\\
%     \Dot{\Bar{x}} &= f(x,u)\\
%     &= \begin{bmatrix}
%         V_x & V_y & V_z & -g\sin \theta & g\sin \theta & \left( \frac{\tau}{m} \right)-g & p & q & r
%     \end{bmatrix}^T
% \end{align}

% % \begin{equation}
% % \label{eqn:9state_nonlin_model}
% % f(x,u)=
% % \begin{bmatrix}
% % V_{x} \\
% % V_{y} \\
% % V_{z} \\
% % -g\sin \theta \\
% % g\sin \theta \\
% % \left( \frac{\tau}{m} \right) -g \\
% % p \\
% % q \\
% % r
% % \end{bmatrix}
% % \end{equation}

% where $\tau$ represents the thrust input in Newtons, $\phi, \theta, \psi$ are the roll, pitch, and yaw angles, and $p, q, r$ are their respective rates of change. We then linearize around the hover position and assume a small-angle approximation to realize our final prediction model.

% Note that our input is 4-dimensional. Therefore, as stated previously, we must define our output to match. We choose to track xyz-position and yaw.
% \begin{equation}
% \label{eqn:outputs}
% y(t) = h(x(t)) = \begin{bmatrix}
% x \\
% y \\
% z \\
% \psi
% \end{bmatrix}
% \end{equation}

% Every reference trajectory we design to be tracked by the output must also match in dimensions and will be defined for the same states.




% \subsection{Predictor}
% \textcolor{red}{SHOULD I ADD GRAVITY? $u(t)-[mg, 0, 0 ,0]$}

% Our look-ahead predictor utilizes the standard closed-form linearized solution to our quadrotor model. However, we can't know the value of $u(\tau)$ during the duration of the lookahead period  $\tau \in [t,t+T]$. We only know its value at the beginning of the period $\tau=t$. Therefore, we hold it constant during the prediction process and move it outside the closed-form solution integral.

% \begin{align}
% \label{eqn:predictor}
%     \xi(t+T) &= e^{ A T }x(t) + \bigl( \int _{0}^T \, e^{ A(T-\tau)}B d\tau \bigr) \cdot u(t)\\
% \label{eqn:predictor2}
%     &= \Tilde{A}x(t) + \Tilde{B} u(t)
% \end{align}

% where $A = \frac{\partial f}{\partial x}(x,u)|_{\Bar{x}^{*}}\in \mathbb{R}^{9\times 9}$ and $B = \frac{\partial f}{\partial u}(x,u)|_{\Bar{x}^{*}} \in \mathbb{R}^{9 \times4}$ are the partial Jacobians with respect to $\Bar{x}$ and $\Bar{u}$ at hover values of $\Bar{x}^{*} = \begin{bmatrix} x & y & z & 0 & 0 & 0 & 0 & 0 & 0 \end{bmatrix}$ and $\Bar{u}^{*}= \begin{bmatrix} mg & 0 & 0& 0\end{bmatrix}$, respectively.

% Using what we've just developed, we can compute the necessary elements for the update equation \eqref{eqn:continuous_time_dynamical_final_NR}. The predicted output becomes $\Hat{y}(t+T) = \psi\bigl(x(t),u(t)\bigr) = h(\xi(t+T))$, and the inverse Jacobian with respect to $u$ renders down to the matrix inverse of the pre-computed integral $B$ in the prediction equation filtered through the output function $h(\cdot)$.

% As is evident from this development, the Newton-Raphson method requires very little knowledge of the system. With our chosen predictor, we need only know the mass of the quadrotor and the gravitational constant. This information is held in the $A$ and $B$ matrices, which are sparse matrices with nonzero elements only equal to $1$, $m$, and $g$.

% In addition, because $A$, $B$, $T$, and $u(t)$ remain constant throughout the program, we can pre-compute and store the constant matrices $\Tilde{A} = e^{ A T }$ and $\Tilde{B} = \int _{0}^T \, e^{ A(T-\tau)}B d\tau$ for use at each iteration of the algorithm. This allows us to create the simplified closed-form predictor \eqref{eqn:predictor2}.
% Doing so also lessens the computational load of this already efficient control method, and creates a predictor which only requires the latest state and input vectors to predict our system state $T$-seconds into the future. This computational efficiency combined with the error bounds demonstrated in Section \ref{sec:newtonraphson derivation} make this tracking controller highly desirable for time-sensitive low-level control in hardware implementations such as the one we showcase in Section \ref{sec:experiments}.
